ADIMA: Abuse Detection In Multilingual Audio

Abusive content detection in spoken text can be addressed by performing Automatic Speech Recognition (ASR) and leveraging advancements in natural language processing. However, ASR models introduce latency and often perform sub-optimally for profane words as they are underrepresented in training corpora and not spoken clearly or completely. Exploration of this problem entirely in the audio domain has largely been limited by the lack of audio datasets. Building on these challenges, we propose ADIMA, a novel, linguistically diverse, ethically sourced, expert annotated and well-balanced multilingual profanity detection audio dataset comprising of 11,775 audio samples in 10 Indic languages spanning 65 hours and spoken by 6,446 unique users. Through quantitative experiments across monolingual and cross-lingual zero-shot settings, we take the first step in democratizing audio based content moderation in Indic languages and set forth our dataset to pave future work.

==> sections/extra.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|c|c| } 
\hline
Language & Train & Test\\ [0.5ex] 
\hline
Hindi & 822 & 369 \\
\hline
Bengali & 822 & 370 \\
\hline
Punjabi & 818 & 367 \\
\hline
Haryanvi & 818 & 366 \\
\hline
Kannada & 819 & 369 \\
\hline
Gujarati & 817 & 362 \\
\hline
Bhojpuri & 762 & 336 \\
\hline
Odia & 814 & 365 \\
\hline
Tamil & 820 & 371 \\
\hline
Malayalam & 819 & 372 \\
\hline
\end{tabular}
\end{center}
\caption{Dataset statistics}
\label{table:data_stats}
\end{table}


\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|c|c| } 
\hline
Language & Unique Users\\ [0.5ex] 
\hline
Hindi & 1200 \\
\hline
Bengali & 679 \\
\hline
Punjabi & 693 \\
\hline
Haryanvi & 264 \\
\hline
Kannada & 469 \\
\hline
Odia & 775 \\
\hline
Bhojpuri & 794 \\
\hline
Gujarati & 232 \\
\hline
Tamil & 1190 \\
\hline
Malyalam & 153 \\
\hline
\end{tabular}
\end{center}
\caption{User statistics. Our dataset comes from different users making it more varied.}
\label{table:user_stats}
\end{table}


\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|l| } 
\hline
Layer & Params\\ [0.5ex] 
\hline
Conv2D & k=3, c=64, s=1 \\
MaxPool2d & k=2, s=2 \\
\hline
\hline
Conv2D & k=3, c=128, s=1 \\
MaxPool2d & k=2, s=2 \\
\hline
\hline
Conv2D & k=3, c=256, s=1 \\
Conv2D & k=3, c=256, s=1 \\
MaxPool2d & k=2, s=2 \\
\hline
\hline
Conv2D & k=3, c=512, s=1 \\
Conv2D & k=3, c=512, s=1 \\
MaxPool2d & k=2, s=2 \\
\hline
\end{tabular}
\end{center}
\caption{VGG Backbone}
\label{table:backbone}
\end{table}
\ramit{We don't need this table, we can directly put this in the training setup section}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/abuse-no-abuse.pdf}
    \caption{Number of samples for \textit{Abusive} and \textit{Non-Abusive} categories for all the languages.}
    \label{fig:category_dist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/unique_users.pdf}
    \caption{Unique users for all the languages.}
    \label{fig:unique_user}
\end{figure}


\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|c|c|c| } 
\hline
Model & Features & \accuracy & \fmacro \\ [0.5ex] 
\hline
\randomguess & - & - & - \\
\hline
LSTM (2-layer-BiDir) & \vgg & 75.06 & 74.84 \\
\hline
GRU (1-layer-BiDir) & \vgg & 76.15 & 76.13 \\
\hline
GRU (2-layer-BiDir) & \vgg & 76.42 & 76.38 \\
\hline
GRU (2-layer-UniDir) & \vgg & 76.42 & 76.41 \\
\hline
\maxpooling & \vgg & 78.05 & 78.01 \\
\hline
\meanpooling & \vgg & \textbf{78.59} & \textbf{78.57} \\
\hline
\maxpooling & \xlsr & 78.86 & 78.76 \\
\hline
\meanpooling & \xlsr & NA & NA \\
\hline
\hline
\maxpooling & \vak & NA & NA \\
\hline
\meanpooling & \vak & NA & NA \\
\hline
\hline

\end{tabular}
\end{center}
\caption{Accuracy and F1 score for different architectures for Hindi}
\label{table:architectures}
\end{table}


\begin{figure*}[h]
\begin{minipage}[b]{0.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/abusive_words_Hindi.pdf}}
  \centerline{(a) Hindi}
\end{minipage}
\begin{minipage}[b]{.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/abusive_words_Kannada.pdf}}
  \centerline{(b) Kannada}
\end{minipage}
\hfill
\begin{minipage}[b]{0.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/abusive_words_Tamil.pdf}}
  \centerline{(c) Tamil}
\end{minipage}
\caption{Histogram of occurence of abusive words in the audios.}
\label{fig:word_stats_per_audi}
\end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/hindi_abuse_word_distribution.pdf}
    \caption{Hindi abuse word distribution for word occurrences greater than 10}
    \label{fig:words_dist}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/duration_hist.pdf}
    \caption{Histogram of durations for all the languages. Majority of audio recordings range from 10 to 25 seconds.}
    \label{fig:duration_hist}
\end{figure}


\begin{figure}
    \begin{subfigure}[b]{0.2\textwidth}
    \includegraphics[width=\linewidth]{figures/Hindi_Yes_duration.pdf}
    \caption{Abusive}
    \label{fig:hindi_duration_dist_yes}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Hindi_No_duration.pdf}
    \caption{Non-Abusive}
    \label{fig:hindi_duration_dist_no}
    \end{subfigure}
    \caption{Hindi audio sample duration distribution in seconds for \textit{abusive} and \textit{non-abusive} audios. Both categories show similar distribution of durations}
\end{figure}

\begin{figure*}[h]
\begin{minipage}[b]{0.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/words_Hindi.pdf}}
  \centerline{(a) Hindi}
\end{minipage}
\begin{minipage}[b]{.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/words_Kannada.pdf}}
  \centerline{(b) Kannada}
\end{minipage}
\hfill
\begin{minipage}[b]{0.33\linewidth}
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/words_Tamil.pdf}}
  \centerline{(c) Tamil}
\end{minipage}
\caption{Frequency of abusive words in the dataset. We plot the count of words which occur more than 5 times in the dataset.}
\label{fig:word_stats}
\end{figure*}

\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|c|c|c|c| } 
\hline
Language & Mean & SD & Min & Max\\ [0.5ex] 
\hline
Hindi & 20.12 & 2.87 & 6.17 & 58.56 \\
\hline
Bengali & 19.98 & 2.29 & 5.90 & 58.30 \\
\hline
Punjabi & 20.06 & 3.29 & 5.03 & 58.47 \\
\hline
Haryanvi & 19.93 & 2.18 & 6.36 & 58.05 \\
\hline
Kannada & 20.23 & 3.75 & 5.29 & 58.02 \\
\hline
Odia & 20.03 & 3.08 & 5.48 & 58.43 \\
\hline
Bhojpuri & 20.12 & 1.7 & 5.24 & 31.62 \\
\hline
Gujarati & 20.21 & 4.02 & 5.01 & 58.45 \\
\hline
Tamil & 20.22 & 3.67 & 6.44 & 58.36 \\
\hline
Malyalam & 20.07 & 2.89 & 5.76 & 57.81 \\
\hline
\end{tabular}
\end{center}
\caption{Duration statistics. Varied durations allows for modelling long and short duration adding variety to our dataset.}
\label{table:duration_stats}
\end{table}


Minorities are usually targeted more than others~\cite{williams2020hate}.

Majority of these datasets use social media platforms like facebook, twitter, reddit, youtube comments etc. as the source for these datasets. 

Audio classification is a well studied area and has been traditionally performed using Gaussian Mixture Models (GMMs)~\cite{zhuang2010real}, Support Vector Machines (SVMs)~\cite{temko2006classification} over hand-crafted features like Mel Frequency Cepstrum Coefficients (MFCCs) or i-vectors~\cite{huang2013blind} \rini{I guess speech would be a better fit for the references here rather than audio in general}. However, with the advancements in deep learning, Convolutional Neural Network (CNN)~\cite{takahashi2016deep},~\cite{hershey2017cnn} and Recurrent Neural Networks (RNN)~\cite{parascandolo2016recurrent},~\cite{xu2018large} solutions have been instrumental in achieving the state-of-the-art results \rini{These references are slightly confusing as the SOTA for audio event detection and speech recognition is different, so we need to establish if we are talking about audio in general or speech}. Audio classification and audio event detection research has been accelerated with the presence of large scale datasets like audio events classification dataset (Audioset)~\cite{hershey2017cnn}, VGG-Sound dataset~\cite{chen2020vggsound}, Urban Sound classification (UrbanSound)~\cite{salamon2014dataset}, Environmental Sound Classification (ESC-50)~\cite{piczak2015esc}, emotion speech and song dataset (RAVDESS)~\cite{livingstone2018ryerson}, , acoustic scene classification and sound event detection~\cite{mesaros2016tut}, ~\cite{foggia2015reliable},~\cite{mesaros2019sound},DCASE~\cite{mesaros2017dcase}, AVE~\cite{tian2018audio}.\vikram{We can get some details about these datasets from this paper https://arxiv.org/pdf/2004.14368.pdf}. 


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/abusive_words_all.pdf}
    \caption{Histogram of occurrence of abusive words in the audios.}
    \label{fig:words_dist}
\end{figure}

\begin{table}[h]
\begin{center}
\begin{tabular}{ |l|c|c|c|c|c| } 
\hline
sr/tg & Hi & Be & Pu & Ha &  Ka\\ [0.5ex] 
\hline
Hi & 77.3 & 69.9/69.8 & 80.2/80.1 & 77.9/76.5 & 79.8/74.7\\
\hline
Be & 72.2/71.8 & 77.9 & 76.9/76.2 & 78.7/78.7 & 75/74.1\\
\hline
Pu & 75.1/75.1 & 75/74.9 & 82.3/82.3 & 78.7/78.2 & 80.9/78.4\\
\hline
Ha & 72.2/72.1 & 74.7/74.3 & 77.7/77.5 & 79.8/79.7 & 76.6/74.6\\
\hline
Ka & 75.9/75.9 & 75.0/74.8 & 80.7/80.6 & 78.9/78.5 & 81.5/79.2\\
\hline
\hline
All & 77.0/77.0 & 75.3/75.1 & 81.5/81.5 & 78.1/77.6 & 81.5/79.2 \\
\hline
\end{tabular}
\end{center}
\caption{Zero-Shot Accuracy and F1 score for different languages}
\label{table:cross_lingual_results}
\end{table}


\begin{table}[h]
\footnotesize
\begin{center}
\begin{tabular}{ |l|c|c|c|c|c| } 
\hline
sr/tg & Hi & Be & Pu & Ka & Ta\\ [0.5ex] 
\hline
Hi & 79.67/79.48 & 78.38/76.95 & 81.47/81.47 & 81.03/79.06 & 80.05/74.67\\
\hline
Be & 78.32/78.32 & 79.73/77.95 & 82.01/82.00 & 78.59/75.23 & 80.32/74.09\\
\hline
Pu & 78.59/78.51 & 78.37/77.08 & 82.01/82.01 & 79.40/77.58 & 79.51/71.00\\
\hline
Ka & 78.32/78.28 & 78.65/77.39 & 82.56/82.42 & 79.67/75.39 & 80.32/74.08\\
\hline
Ta & 77.23/77.13 & 77.29/76.00 & 83.38/83.38 & 79.40/77.10 & 80.59/73.29\\
\hline
\hline
All & NA & NA & NA & NA & NA \\
\hline
\end{tabular}
\end{center}
\caption{Zero-Shot Accuracy and F1 score for different languages}
\label{table:cross_lingual_results}
\end{table}

\subsection{Problem Formulation} We consider the task of classifying audio recording $x$ into $c$ $\in$ \{\textit{abusive}, \textit{non-abusive}\} categories. We extract features from the audio recording $x$ using feature backbones $\phi$. We experiment with \vgg and \wavvec backbones which are based on CNNs over log-mel spectogram and Transformer architecture over raw audio respectively. The features are then aggregated using aggregator function $\theta$ and are passed through a fully connected classifier for classification. We perform the analysis under monolingual and cross-lingual settings for exploring cross-learning between the languages.


ShareChat does not record the user conversations to maintain the user privacy. However, recordings are done for a short duration (5 seconds to 60 seconds) after multiple users report an instance of abusive behaviour and are shared with the content moderation team for review. \vikram{Debdoot, this can be a little sensitive issue. We need to be more careful about writing this.}

==> sections/rebuttal_r1.tex <==

\noindent\textbf{Title of paper:} We thank the reviewer for thoughtful and thorough review. Our work is focused on detection of abuse in spoken audio recordings and we agree with the reviewer that “profanity detection” can be confusing to readers. We will modify the title of our work to \textit{"ADIMA: Abuse Detection in Multilingual Audio"}. We hope that the revised title is more coherent with the remaining draft and will help in avoiding future confusions. Thanks again for your feedback.
\vfill\pagebreak


==> sections/rebuttal_r2.tex <==
We thank the reviewer for thoughtful review and helpful suggestions. We are glad that the reviewer found our work interesting. Studying the impact of prosody, recipient and context is a great research direction and we will consider them in our future work. 

\noindent\textbf{Annotation Guidelines:} For this study, we considered the presence of swear, cuss and abusive words/phrases as profanity. For each language, we hired three annotators who were native speakers of that language. We leveraged their expertise to identify the audios which contain words/phrases that are identified as offensive. The profane words/phrases were catalogued and reviewed to make sure that there is consensus among the three reviewers.  

\noindent\textbf{Inter-Annotator agreement scores:} We measured the inter-annotator agreement using Cohen's Kappa and observed an average score of 0.88 which indicates high degree of agreement amongst the three annotators. Cohen's Kappa varied from 0.77 to 1.0 across different languages, indicating the variation in complexity across languages for the same task. The final decision was taken by a fourth expert annotator in case of disagreements. Section 3.2 in our paper discusses this in more detail. 
 
\noindent\textbf{VGG performance:} VGG model was trained over the AudioSet dataset which contains audio clips extracted from YouTube videos and annotated with 527 sound categories like music, speech, vehicle, singing, gargling etc. The high performance of VGG (trained over AudioSet dataset) is surprising as this model was trained to discriminate between different sounds instead of understanding human speech. One possible explanation could be that there exists correlation between profanity and fundamental audio properties like pitch/frequency which are captured by the VGG features. For instance, generally, humans are agitated while using abusive words and may use higher pitch and amplitude. However, a further detailed study is required to understand and establish these correlations. 

\noindent\textbf{Figures readability:} Thanks for highlighting this problem. We will update the figures to make them compatible for grey-scale reading.

\vfill\pagebreak



==> sections/rebuttal_r3.tex <==
We thank the reviewer for a comprehensive review. 

\noindent\textbf{Evaluation using conventional methods:} Thank you for pointing us to the work by Yousefi et al. Their work is contemporary to our work, thus we were not aware about their work at the time of our investigation and submission. However, for adequate benchmarking, we additionally report weighted accuracy (\wacc), area under the receiver operating characteristic (ROC) curve (\auc) and area under the precision-recall curve (\aucpr) for our best performing pooling models in Table~\ref{table:em_architectures}. Our weighted accuracy (\wacc) is closer to unweighted accuracy (\accuracy) highlighting the balance of our models for both classes. Due to time and compute constraint, we could not complete the additional metrics for all the other models. However, we will strive to accommodate them in the next version of our draft. 


\setcounter{table}{0}
\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{ llccccl } 
\hline
Backbone & Model & \accuracy & \fmacro & \wacc & \auc &\aucpr \\ [0.5ex] 
\hline
\multirow{2}{*}{\vgg} & \maxpooling  & 78.05 & 78.01 & 78.01 & 0.84 & 0.85 \\
& \meanpooling & 78.59 & 78.57 & 78.55 & 0.85 & 0.86\\
\hline
\multirow{2}{*}{\xlsr} & \maxpooling & 76.96 & 76.90 & 76.93 & 0.84 & 0.84 \\
& \meanpooling & 77.51 & 77.34 & 77.44 & 0.83 & 0.85\\
\hline
\multirow{2}{*}{\vak} & \maxpooling & 79.13 & 79.03 & 79.08 & 0.85 & 0.86\\
& \meanpooling & 78.86 & 78.69 & 78.80 & 0.85 & 0.85\\
\hline
\multirow{2}{*}{\clsril} & \maxpooling &  \textbf{79.67} & \textbf{79.48} & \textbf{79.60} & 0.86 & 0.86\\
& \meanpooling & 78.59 & 78.59 & 78.59 & 0.86 & 0.84\\
\hline

\end{tabular}
\end{center}
\caption{Accuracy (\accuracy), Macro F1 (\fmacro), Weighted Accuracy (\wacc), Area under ROC curve (\auc) and Area under Precision-Recall curve (\aucpr) for different architectures and backbones for Hindi.}
\label{table:em_architectures}
\end{table}

\noindent\textbf{Annotation Guidelines:} For this study, we considered the presence of swear, cuss, offensive and abusive words/phrases for classification into abusive audios. For each language, we leveraged the expertise of three annotators who were native speakers of the language to identify the presence of words/phrases which are considered offensive. The abusive words/phrases were also catalogued and reviewed to make sure there is consensus among the three reviewers. We measured the inter-annotator agreement using Cohen's Kappa and observed an average score of 0.88 which indicates high degree of agreement amongst the three annotators. Cohen's Kappa varied from 0.77 to 1.0 across different languages, indicating the variation in complexity across languages for the same task. The final decision was taken by a fourth expert annotator in case of disagreements. 

\noindent\textbf{Model Architecture:} In \maxpooling and \meanpooling models, we perform the respective pooling operation across the temporal dimension of the audio features before passing them through the classifier. After pooling, each audio gets represented by 512 dimensional feature vector. This feature vector is then passed through the binary classifier which consists of three fully connected layers ($512\rightarrow256\rightarrow128\rightarrow2$) with ReLU activation and 0.1 dropout. For \lstm/\gru, instead of pooling operation, we model the temporal information using a bidirectional \lstm/\gru layer before passing the output of the final time step through the binary classifier. We will add these details in Section 4.3 in the next version of our draft.


\noindent\textbf{Figures 1(c-d) for other languages:} Considering financial constraints, we annotated the abusive words/phrases present in the audio for only three languages. This helped us to perform the initial study and understand the distribution of our dataset. Since the distribution of abusive words for the three languages was diverse, we annotated the remaining languages with the presence/absence of abusive words only to save time and budget. We will try to collect detailed annotations for other languages also if our budget permits. 

\noindent\textbf{LSTM/GRU results:} We experimented with \lstm/\gru for other backbones also but similar to \vak, results did not improve significantly as compared to the \meanpooling and \maxpooling results. From Table~\ref{table:re_architectures}, we can note that pooling models  are competitive or outperform \lstm/\gru. Due to the lack of significant performance improvement and space constraints, we did not include them in the draft. 

\begin{table}[h!]
\begin{center}
\small
\begin{tabular}{ llrr } 
\hline
Backbone & Model & \accuracy & \fmacro & \\ [0.5ex] 
\hline
\multirow{4}{*}{\vgg} & \maxpooling  & 78.05 & 78.01 \\
& \meanpooling & 78.59 & 78.57\\
& \gru & 78.57 & 78.56\\
& \lstm & 77.77 & 77.71\\
\hline
\multirow{4}{*}{\xlsr} & \maxpooling & 76.96 & 76.90 \\
& \meanpooling & 77.51 & 77.34 \\
& \gru & 77.49 & 77.31 \\
& \lstm & 77.24 & 77.23\\
\hline
\multirow{4}{*}{\vak} & \maxpooling & 79.13 & 79.03 \\
& \meanpooling & 78.86 & 78.69 \\
 & \gru & 77.50 & 77.50 \\
& \lstm  & 77.10 & 77.02\\
\hline
\multirow{4}{*}{\clsril} & \maxpooling &  \textbf{79.67} & \textbf{79.48} \\
& \meanpooling & 78.59 & 78.59 \\
& \gru & 75.34 & 75.23\\
& \lstm & 70.19 & 69.53\\
\hline
\end{tabular}
\end{center}
\caption{Accuracy (\accuracy) and Macro F1 (\fmacro) for different architectures and backbones for Hindi.}
\label{table:re_architectures}
\end{table}

\noindent\textbf{Him-4200 results:} Even though \vak model is fine-tuned over Hindi data, it did not outperform the multilingual \clsril model. Thus, for further study, we chose multilingual and language-agnostic models as the backbone and studied the performance for multiple languages across monolingual, cross lingual and combination of language settings. 

\noindent\textbf{Dataset Release:} We apologize for this unintentional delay. Our understanding was that dataset is released with camera ready version. We have now uploaded our codebase and dataset:  

\url{https://bit.ly/3FivgBP}

\noindent\textbf{Captions and references:} Thanks for pointing this out. We will address them in the next version of our draft.



% \begin{table}[t]
% \scriptsize
% \begin{center}
% \begin{tabular}{ llrrrrr } 
% \hline
% Backbone & Model & \accuracy & \fmacro & \wacc & \auc &\aucpr \\ [0.5ex] 
% \hline
% \multirow{4}{*}{\vgg} & \maxpooling  & 78.05 & 78.01 & 78.01 & 84.40 & 84.60 \\
% & \meanpooling & 78.59 & 78.57 & 78.55 & 84.47 & 86.10\\
% & \gru & 77.78 & 77.62 & - & -\\
% & \lstm & 77.24 & 76.89 & - & - \\
% \hline
% \multirow{4}{*}{\xlsr} & \maxpooling & 76.96 & 76.90 & 76.93 & 83.68 & 84.18 \\
% & \meanpooling & 77.51 & 77.34 & 77.44 & 82.85 & 85.31\\
% & \gru & 76.96 & 76.94 & - & -\\
% & \lstm & 77.24 & 77.20 & - & -\\
% \hline
% \multirow{4}{*}{\vak} & \maxpooling & 79.13 & 79.03 & 79.08 & 84.81 & 85.45\\
% & \meanpooling & 78.86 & 78.69 & 78.80 & 84.54 & 85.13\\
%  & \gru & 77.50 & 77.50 & - & -\\
% & \lstm  & 77.10 & 77.02 & - & -\\
% \hline
% \multirow{4}{*}{\clsril} & \maxpooling &  \textbf{79.67} & \textbf{79.48} & 79.60 & 85.69 & 86.24\\
% & \meanpooling & 78.59 & 78.59 & 78.59 & 86.27 & 84.14\\
% & \gru & 78.05 & 77.99 & - & -\\
% & \lstm & 68.56 & 68.51 & - & -\\
% \hline

% \end{tabular}
% \end{center}
% \caption{Accuracy (\accuracy), Macro F1 (\fmacro), Weighted Accuracy (\wacc), Area under ROC curve (\auc) and Area under Precision-Recall curve (\aucpr) for different architectures and backbones for Hindi.}
% \label{table:re_architectures}
% \end{table}
